Joint Study of Above Ground Biomass and Soil Organic Carbon for Total Carbon Estimation using Satellite Imagery in Scotland

Land Carbon verification has long been a challenge in the carbon credit market. Carbon verification methods currently available are expensive, and may generate low-quality credit. Scalable and accurate remote sensing techniques enable new approaches to monitor changes in Above Ground Biomass (AGB) and Soil Organic Carbon (SOC). The majority of state-of-the-art research employs remote sensing on AGB and SOC separately, although some studies indicate a positive correlation between the two. We intend to combine the two domains in our research to improve state-of-the-art total carbon estimation and to provide insight into the voluntary carbon trading market. We begin by establishing baseline model in our study area in Scotland, using state-of-the-art methodologies in the SOC and AGB domains. The effects of feature engineering techniques such as variance inflation factor and feature selection on machine learning models are then investigated. This is extended by combining predictor variables from the two domains. Finally, we leverage the possible correlation between AGB and SOC to establish a relationship between the two and propose novel models in an attempt outperform the state-of-the-art results. We compared three machine learning techniques, boosted regression tree, random forest, and xgboost. These techniques have been demonstrated to be the most effective in both domains.

==> notes.tex <==
Summary Table for AGB - summary of literature - done
SOC summary table - done

Spatial Characteristics of carbon maps - done
Discussion - write something, maybe findings or insights





Maybe maybe not 
\newline
There are numerous papers obtaining the state-of-the-art results in the domain of remote sensing for carbon estimation. Two of which present the most recent findings in SOC estimation and AGB estimation. Zhou et al. \citep{zhou_2020} suggested that soil carbon content could be estimated using Sentinel 1, Sentinel 2, and Digital Elevation Map. Li et al. \citep{li_2020} estimated above-ground biomass in forests using LandSat 8 and Sentinel 1A.  
Our implementation is evaluated using three machine learning techniques: BRT, RF, and XGB. Section \ref{sec:exp-models} details the models with various input variables. The choice of machine learning techniques and input data for our baseline is motivated by prior research. We obtain comparable results for our study site to use as a baseline for evaluating state-of-the-art performances.



In this section, we investigate the indirect relationship between AGB, SOC and SOC Density. The state-of-the-art remote sensing carbon research mainly focuses on estimating AGB or estimating SOC separately \citep{zhou_2020}\citep{li_2020}. However, with recent development in climate change and the rise of the voluntary carbon market sparks interests for total carbon prediction. Previous studies suggest possible correlation between AGB and SOC with strong evidence that one influences the other \citep{total-2} \citep{Gebeyehu2019} \citep{multivariate_loess_plateau_2018}. The domains of AGB and SOC should be treated as one ecosystem, but pioneering research in remote sensing has only aggregated research in each domain and failed to address the indirect relationship between AGB and SOC. We therefore present a novel approach in Remote Sensing Total Carbon Estimation that takes into account the indirect relationship between AGB and SOC.
\newline\newline
We have explored in previous sections the effect of SOC predictors on AGB and vice versa. By including DEM data in AGB estimation models, we were able to improve the state-of-the-art results by $R^2$ = 8.82\% (Comparing BRT model B and model F). Following this novel finding, we now propose two new models - Model G and Model H which consists of target variables, meaning we use AGB as a predictor for SOC and vice versa. The details of the model can be found in section \ref{subsec:final_model}.

